Computationally Tractable Riemannian Manifolds for Graph Embeddings

Representing graphs as sets of node embeddings in certain curved Riemannian manifolds has recently gained momentum in machine learning due to their desirable geometric inductive biases, e.g., hierarchical structures benefit from hyperbolic geometry. However, going beyond embedding spaces of constant sectional curvature, while potentially more representationally powerful, proves to be challenging as one can easily lose the appeal of computationally tractable tools such as geodesic distances or Riemannian gradients. Here, we explore computationally efficient matrix manifolds, showcasing how to learn and optimize graph embeddings in these Riemannian spaces. Empirically, we demonstrate consistent improvements over Euclidean geometry while often outperforming hyperbolic and elliptical embeddings based on various metrics that capture different graph properties. Our results serve as new evidence for the benefits of non-Euclidean embeddings in machine learning pipelines.

==> Makefile <==
ifndef V
Q = @
Q_LATEX = sh -c 'echo -e "   " `echo $$(basename "$$0") | tr a-z A-Z`"\t$${!\#/..\/..\//}"; ! "$$0" "$$@" | grep -A5 -E "^[^ ]+:[0-9]+:"'
Q_OTHER = sh -c 'echo -e "   " `echo $$(basename "$$0") | tr a-z A-Z`"\t$${!\#/..\/..\//}"; "$$0" "$$@" >/dev/null'
endif

PDFLATEX = pdflatex
BIBTEX = bibtex

.PHONY: matrix-manifolds.pdf
matrix-manifolds.pdf:
	$(Q) $(Q_LATEX) $(PDFLATEX) -interaction=nonstopmode -file-line-error matrix-manifolds.tex
	$(Q) $(Q_OTHER) $(BIBTEX) matrix-manifolds
	$(Q) $(Q_LATEX) $(PDFLATEX) -interaction=nonstopmode -file-line-error matrix-manifolds.tex
	$(Q) $(Q_LATEX) $(PDFLATEX) -interaction=nonstopmode -file-line-error matrix-manifolds.tex

.PHONY: clean
clean:
	rm -f *.log *.lot *.lof *.blg *.bbl *.out *.toc *.aux *.thm *.idx *.ilg *.nlo *.nls &>/dev/null || true


==> src/sections/software.tex <==
\section*{Software and Data}

